Multimodal Dialogue State Tracking

Designed for tracking user goals in dialogues, a dialogue state tracker is an essential component in a dialogue system. However, the research of dialogue state tracking has largely been limited to unimodality, in which slots and slot values are limited by knowledge domains (e.g. restaurant domain with slots of restaurant name and price range) and are defined by specific database schema. In this paper, we propose to extend the definition of dialogue state tracking to multimodality. Specifically, we introduce a novel dialogue state tracking task to track the information of visual objects that are mentioned in video-grounded dialogues. Each new dialogue utterance may introduce a new video segment, new visual objects, or new object attributes, and a state tracker is required to update these information slots accordingly. We created a new synthetic benchmark and designed a novel baseline, Video-Dialogue Transformer Network (VDTN), for this task. VDTN combines both object-level features and segment-level features and learns contextual dependencies between videos and dialogues to generate multimodal dialogue states. We optimized VDTN for a state generation task as well as a self-supervised video understanding task which recovers video segment or object representations. Finally, we trained VDTN to use the decoded states in a response prediction task. Together with comprehensive ablation and qualitative analysis, we discovered interesting insights towards building more capable multimodal dialogue systems.

==> content/dataset.tex <==
\section{DVD-DST Benchmark}

Since there is no prior benchmarks that are suitable for MM-DST, we developed a synthetic benchmark of video-grounded dialogues based on the generation procedure of DVD \citep{le-etal-2021-dvd}. 
The benchmark, denoted DVD-DST, contains all video segment annotations and object state annotations for each dialogue turn. 
We extended the dialogue generation procedure of \citep{le-etal-2021-dvd} to include state annotation at each dialogue turn. 
Different from \cite{le-etal-2021-dvd}, we chose to generate dialogue data based on an extended CATER video split \citep{shamsian2020learning} rather than the original CATER video data \citep{Girdhar2020CATER}. 
The extended CATER videos \citep{shamsian2020learning} includes additional annotations of bounding box boundaries of each visual object in video frames. 
This annotation facilitates our experiments later with model of perfect object perception, i.e. $P(o_j | \mathcal{V}, \omega) \approx 1$. 
Based on the CATER universe, we defined a total of 6 types of slots: including slots of attributes ``size'', ``color'', ``material'', and ``shape'', and 2 slots for $s_\mathrm{start}$ and $s_\mathrm{end}$.
Since each CATER video contains only fixed object set, $s_\mathrm{start}$ and $s_\mathrm{end}$ are defined per turn rather than per dialogue. 
The synthetic dataset allowed us to control any data bias as each object is synthesized by random slot attributes and each dialogue turn is designed to involve randomly sampled objects and video segments.
A comparison of statistics of DVD-DST and prior DST benchmarks can be seen in Table \ref{tab:data}. 



==> content/related_work.tex <==
\section{Related Work}

Our work is related to research domains: dialogue state tracking and visually-grounded dialogues.

\subsection{Dialogue State Tracking}
Dialogue State Tracking (DST) research aims to develop models that can track essential information conveyed in dialogues between a dialogue agent and human (defined as hidden information state by \cite{YOUNG2010150} or belief state by \cite{mrksic2017neuralbelief}). 
DST research has evolved largely within the domain of task-oriented dialogue systems.
DST is often designed in a modular dialogue systems and preceded by a Natural Language Understanding (NLU) component. 
NLU learns to label sequences of dialogue utterances and provides a tag for each word token (often in the form of In-Out-Begin representations) \citep{kurata-etal-2016-leveraging, shi-etal-2016-recurrent, rastogi2017ScalableMD}. 
To avoid credit assignment problems and streamline the modular designs, NLU and DST have been integrated into a single module \citep{mrksic2017neuralbelief, xu2018end, zhong-etal-2018-global}. 
These DST approaches can be roughly categorized into two types: fixed-vocabulary or open-vocabulary. 
Fixed-vocabulary approaches are designed for classification tasks which assume a fixed set of \emph{(slot, value)} candidates and directly retrieve items from this set to form dialogue states during test time \citep{henderson2014RobustDS, ramadan2018large, lee2019sumbt}.
More recently, we saw more approaches toward open-vocabulary strategies which learn to generate candidates based on input dialogue context \citep{lei2018sequicity, gao2019dialog, wu-etal-2019-transferable, Le2020Non-Autoregressive}. 
Our work is more related to open-vocabulary DST, but we essentially redefined the DST task with multimodality. 
Based on our literature review, we are the first to formally extend DST and bridge the gap between traditional task-oriented dialogues and multimodal dialogues. 

\subsection{Visually-grounded Dialogues}

A novel challenge to machine intelligence,  the intersection of vision and language research has expanded considerably in the past few years. 
Earlier benchmarks test machines to perceive visual inputs,  and learn to generate captions \citep{farhadi2010every, lin2014microsoft, rohrbach2015dataset}, ground text phrases and objects \citep{kazemzadeh2014referitgame, plummer2015flickr30k}, and answer questions about the visual contents \citep{antol2015vqa, zhu2016visual7w, jang2017tgif, lei-etal-2018-tvqa}. 
An orthogonal development from this Visual Question Answering problems, we noted recent work that targets vision-language in dialogue context, in which an image or video is given and the dialogue utterances are centered around its visual contents \citep{de2017guesswhat, das2017visual, visdial_eval, hori2019avsd, thomason:corl19}. 
Recent work has addressed different challenges in visually-grounded dialogues, including multimodal integration \citep{}, cross-turn dependencies \citep{}, and video understanding \citep{}. 
Our work is more related to the challenge of visual object reasoning \citep{}. 
However, the prior approaches are not well designed to track objects and maintain a recurring memory or state of these objects from turn to turn. 
This challenge becomes more obvious when a dialogue involves multiple objects of similar characters or appearance.
We directly tackles this challenge as we formulated a novel multimodal state tracking task and leveraged the research development from DST in task-oriented dialogue systems. 

